Weakest Precondition Reasoning for Expected Run-Times of Probabilistic Programs

This paper presents a wp-style calculus for obtaining bounds on the expected run-time of probabilistic programs. Its application includes determining the (possibly infinite) expected termination time of a probabilistic program and proving positive almost-sure termination - does a program terminate with probability one in finite expected time? We provide several proof rules for bounding the run-time of loops, and prove the soundness of the approach with respect to a simple operational model. We show that our approach is a conservative extension of Nielson's approach for reasoning about the run-time of deterministic programs. We analyze the expected run-time of some example programs including a one-dimensional random walk and the coupon collector problem.

==> Makefile <==
.PHONY: default clean distclean


default: main.pdf


main.pdf: *.tex literature.bib ./pics/*.tex 
	pdflatex main && \
	bibtex main && \
	pdflatex main && \
	pdflatex main


clean:
	rm -f *.aux *.log *.bbl *.blg *~ main.pdf *.out *.synctex.gz

distclean: clean
	rm -f main.pdf


==> app-banach.tex <==





\subsection{Proof of Theorem \ref{thm:expratio-semimetric}}
\label{sec:proof-thm-expratio-semimetric}

\begingroup
\def\thetheorem{\ref{thm:expratio-semimetric}}
\begin{theorem}
$\expRatiosymbol$ is a $(\E,\, {\preceq})$--semimetric on $\Eefin$.
\end{theorem}
\addtocounter{theorem}{-1}
\endgroup



\begin{proof}
First we show that $\expRatiosymbol$ complies with the axiom of coincidence:
\begin{align*}
&\expRatio{f}{g} ~=~ \zero\\
~\Longleftrightarrow~&\lambda \sigma.\: \left| \ln\left(\frac{f(\sigma)}{g(\sigma)} \right) \right| ~=~ \zero\tag{Definition \ref{def:expratio}}\\
~\Longleftrightarrow~&\forall \sigma\in\States\colon \left| \ln\left(\frac{f(\sigma)}{g(\sigma)} \right) \right| ~=~ 0\\
~\implies\;&\forall \sigma\in\States\colon\ln\left(\frac{f(\sigma)}{g(\sigma)} \right) ~=~ 0 \tag{$|0| = 0$}\\
~\Longleftrightarrow~&\forall \sigma\in\States\colon \frac{f(\sigma)}{g(\sigma)} ~=~ 1 \tag{$\ln(x) = 0$ iff $x = 1$}\\
~\Longleftrightarrow~&\forall \sigma\in\States\colon f(\sigma) ~=~ g(\sigma) \tag{$g(\sigma) \neq 0$}\\
~\Longleftrightarrow~&f ~=~ g
\end{align*}
Next we show that $\expRatiosymbol$ is symmetric. For that consider the following:
\belowdisplayskip=0\baselineskip
\begin{align*}
	\expRatio{f}{g} ~=~ &\lambda \sigma.\: \left| \ln\left(\frac{f(\sigma)}{g(\sigma)} \right) \right|\tag{Definition \ref{def:expratio}}\\
	~=~ &\lambda \sigma.\: \left| \ln\big(f(\sigma)\big) - \ln\big(g(\sigma)\big) \right|\tag{$\ln(\nicefrac x y) = \ln(x) - \ln(y)$}\\
	~=~ &\lambda \sigma.\: \left| \ln\big(g(\sigma)\big) - \ln\big(f(\sigma)\big) \right|\tag{$|x-y| = |y-x|$}\\
	~=~ &\lambda \sigma.\: \left| \ln\left(\frac{g(\sigma)}{f(\sigma)} \right) \right|\tag{$\ln(\nicefrac x y) = \ln(x) - \ln(y)$}\\
	~=~ &\expRatio{f}{g}\tag{Definition \ref{def:expratio}}
\end{align*}
\qed
\end{proof}

==> leftover.tex <==
In the following we will develop a denotational semantics for reasoning about expected execution times of probabilistic programs. 
For that we first recall some preliminaries.




\subsection{Preliminaries}

Denotational semantics usually builds upon the concept of complete partial orders and continuous functions---two notions we briefly recall:
%
%
\begin{definition}[Complete Partial Orders \cite{cpos}]
\label{def:cpo}
Let $D$ be some set\footnote{This set is usually called the \emph{domain}.} and ${\sqsubseteq} \subseteq D \times D$. Then $(D,\, {\sqsubseteq})$ is a \textbf{partial order} (\textbf{CPO} for short) iff $\sqsubseteq$ is
\begin{enumerate}
\item reflexive, i.e.~for all $d \in D$ holds $d \sqsubseteq d$,
\item transitive, i.e.~for all $d_1, d_2, d_3\in D$ holds: if $d_1 \sqsubseteq d_2$ and $d_2 \sqsubseteq d_3$ then also $d_1 \sqsubseteq d_3$, and
\item antisymmetric, i.e.~for all $d_1,d_2 \in D$ holds: if $d_1 \sqsubseteq d_2$ and $d_2 \sqsubseteq d_1$ then $d_1 = d_2$.
\end{enumerate}
We write $d_1 \sqsubset d_2$ iff $d_1 \sqsubseteq d_2$ and $d_1 \neq d_2$.

A partial order $\sqsubseteq$ is called \textbf{complete} iff every subset $S \subseteq D$ has a supremum.\footnote{Dually every subset also has an infimum.}
The least and the greatest element of a complete partial order are referred to as the \textbf{bottom element} and the \textbf{top element}, respectively.\footnote{The least and the greatest element of a complete partial order $(D,\, {\sqsubseteq})$ always exist as these are given by $\sup D$ and $\sup \emptyset$, respectively.}
\end{definition}
%
%
%
%
\begin{definition}[Scott--Continuity \cite{scott-continuity}]
Let $(D,\, {\sqsubseteq})$ be a complete partial order and $F\colon D \rightarrow D$. 
Then $F$ is called scott--continuous or simply \textbf{continuous} iff for all subsets $S \subseteq D$ holds
\begin{align*}
F(\sup S) ~=~ \sup F(D)~,
\end{align*}
where $F(D) = \{f(d) ~|~ d \in D\}$.
Notice that every continuous function $F$ is also necessarily \textbf{monotonic}, i.e.\
\begin{align*}
	\textnormal{$F$ continuous} ~\implies~ \big(\forall d_1, d_2\mydot d_1 \sqsubseteq d_2 \implies F(d_1) \sqsubseteq F(d_2) \big)~.
\end{align*}
\end{definition}
%
%
An important and widely used theorem in the field of denotational semantics and computation in general is the Kleene Fixed Point Theorem---a theorem restated and reproven in many different flavors \cite{folktale}.
%
%
\begin{theorem}[Kleene Fixed Point Theorem \cite{folktheorem}]
\label{thm:kleeneFP}
Let $(D,\, {\sqsubseteq})$ be a complete partial order with bottom element $\bot \in D$ and top element $\top \in D$ and let $F\colon D \rightarrow D$ be continuous.
Then $F$ has at least one fixed point and its least fixed point $\lfp F$ and its greatest fixed point $\gfp F$ are given, respectively, by
\begin{align*}
\lfp F ~=~ \sup_{n \in \mathbb N} F^n(\bot) \qquad \text{and} \qquad \gfp F ~=~ \sup_{n \in \mathbb N} F^n(\top)~.
\end{align*}
\end{theorem}
%
%
A more general version of the Kleene Fixed Point Theorem is the so called Tarski--Kontorovich Principle:
%
%
\begin{theorem}[Tarski--Kantorovich Principle \cite{tarski-kantorovich}]
\label{thm:tarski-kantorovich}
	Let $(D,\, \sqsubseteq)$ be a complete partial order, let $F\colon D \To D$ be continuous, and let $b \in D$ such that $b \sqsubseteq F(b)$.
	Then $F$ has a fixed point in the set $\{d \in D ~|~ b \sqsubseteq d\}$ and the least fixed point of $F$ in this set is given by
	\begin{align*}
		\sup_{n \in \Nats} F^n(b)~.
	\end{align*}
	Dually, let $c \in D$ such that $F(c) \sqsubseteq c$.
	Then $F$ has a fixed point in the set $\{d \in D ~|~ d \sqsubseteq c\}$ and the greatest fixed point of $F$ in this set is given by
	\begin{align*}
		\inf_{n \in \Nats} F^n(c)~.
	\end{align*}
\end{theorem}
%
%
As a last preliminary note, we recall a sufficient condition for a point to be above the least fixed point and below the greatest fixed point, respectively:
%
%
\begin{lemma}[Park's Lemma \cite{prefp}]
\label{lem:park}
Let $(D,\, {\sqsubseteq})$ be a complete partial order, let $F\colon D \rightarrow D$ be continuous, and let $d \in D$.
Then
\begin{enumerate}
\item $F(d) \sqsubseteq d ~\implies~  \lfp F \sqsubseteq d$, and
\item $d \sqsubseteq F(d) ~\implies~ d \sqsubseteq \gfp F$.
\end{enumerate}
\end{lemma}
%
%




\subsection{The Expected Execution Time Transformer}

In order to develop a denotational semantics for expected execution times based on complete partial orders and continuous functions, we first need to define a proper domain.
We will use the set of so called \emph{expectations} \`{a} la McIver \& Morgan \cite{MM}.
An expectation is hence simply a function mapping a program state to a positive real or $\infty$.
A more intuitive term for an expectation would be: \emph{random variable}.
In order to avoid any confusion and since we want to reason about expected execution times of programs, we will simply speak of \emph{execution times}.
The reason that we think of execution times as a mapping from program states to reals is that the expected execution time of a program may depend on the initial state the program is started in.
Formally, we have:
%
%
\begin{definition}[Execution Times]
\label{def:expectations}
The set of execution times $\E$ is defined as
\begin{align*}
\E ~=~ \left\{f~\middle|~f\colon \States \rightarrow \Rposinf\right\}~.
\end{align*}
The order ${\preceq} \subseteq \E \times \E$ on $\E$ is defined as
\begin{align*}
f \preceq g ~\Longleftrightarrow~ \forall \sigma\in\States\mydot f(\sigma) \leq g(\sigma)~.
\end{align*}
Accordingly, we write $f \prec g$ iff $f \preceq g$ and $f \neq g$.
\end{definition}
%
%
The order we have defined on the set of expectations is the pointwise less or equal. 
With this ordering relation, we can indeed show that $(\E,\, {\preceq})$ is a complete partial order.
%
%
\begin{theorem}
\label{thm:cpo}
$(\E,\, {\preceq})$ is a complete partial order with bottom element $\zero\colon \sigma \mapsto 0$ and top element $\infinity\colon \sigma \mapsto \infty$.
\end{theorem}
%
%
%
%
\begin{proof}
	See Appendix \ref{sec:proof-thm-cpo}.
	\qed
\end{proof}
%
%
\TODO{In the remainder use macro $\backslash\texttt{ctert}\{\ldots\}$ for constant running times.}

On top of the above domain and the complete partial order we can now define a denotational semantics for expected execution times of probabilistic programs in terms of expected execution time transformers.
Such a transformer takes a program $C$ and an execution time $f$, the so called \emph{post--execution time}, and transforms it into another execution time $g$, the so called \emph{pre--execution time}.
The post--execution time can be thought of as an execution time that must be accounted for after $C$ is executed. 
Recall that execution times are functions mapping program states to reals. 
The post--execution time can hence be though of as being evaluated in the final state that is reached after $C$'s termination.

The pre--execution time $g$ can now be thought of in the following way: 
When starting the program $C$ in initial state $\sigma$, then $g(\sigma)$ is the expected execution time of the program $C$ plus $p \cdot f(\tau)$ where $\tau$ is some final state that is reached with probability $p$ after executing the program $C$ on input $\sigma$.

At first glance the concept of a post--execution time might seem unnecessary, but it enables us express the joint expected execution time of two sequentially composed programs in a compositional way. 
Formally, our transformer is defined as follows:
%
%
\begin{definition}[The Expected Execution Time Transformer $\boldeetsymbol$]% and the Liberal Expected Execution Time Transformer $\boldleetsymbol$]
\label{def:eet-rules}
The expected execution time transformer $\eetsymbol\colon \appProgs \times \E \rightarrow \E$ 
%and the liberal expected execution time transformer $\leetsymbol\colon \appProgs \times \E \rightarrow \E$ are 
is defined inductively on the program structure according to the rules given in Table \ref{table:eet-rules}.
\end{definition}
%
%
\begin{table}[t!]
\begin{center}
\renewcommand{\arraystretch}{1.5}
\begin{tabular}{l@{\qquad}l}
\hline\hline
$~\boldsymbol{\quad\qquad C~}$ & $\boldsymbol{\boldeetsymbol\left[C\right]\left(f\right)}~$\\
\hline\hline
$\quad\qquad~\EMPTY$ & $f$\\
%
$\quad\qquad~\SKIP$ & $\ctert{1} + f$\\
%
$\quad\qquad~\APPASSIGN x \mu$ & $\ctert{1} + \lambda \sigma\mydot
\Exp{\pexprdeno{\mu}(\sigma)}{\lambda v.\: f\subst{x}{v}}$\\
%
% $\quad\qquad~\APPASSIGN x \mu$ & $\ctert{1} + \sum_{v} \Big(\probof{\mu}{v}
% \cdot f\subst{x}{v}\Big)$\\
%
$\quad\qquad~\COMPOSE{C_1}{C_2}$ & $\eet{C_1}{\eet{C_2}{f}}$\\
%
$\quad\qquad~\!\!\NDCHOICE{C_1}{C_2}$ & $\max\{\eet{C_1}{f},\,
\eet{C_2}{f}\}\qquad\quad\,$\\
%
$\quad\qquad~\ITE{\pguard}{C_1}{C_2}$ & $\ctert{1} + \probof{\pguard}{\true}
\cdot \eet{C_1}{f} + \probof{\pguard}{\false} \cdot \eet{C_2}{f}$\\
%
$\quad\qquad~\WHILEDO{\pguard}{C'}$ & $\lfp X\mydot \ctert{1} + \probof{\pguard}{\false} \cdot f + \probof{\pguard}{\true} \cdot \eet{C'}{X}$
\end{tabular}
\end{center}
\hrule
\vspace{1\baselineskip}
\caption{Rules for the expected execution time transformer $\eetsymbol$. $\lfp$
  stands for the least fixed point operator.}
%\label{table:eet-rules}
\end{table}
%
%
We can prove that or transformer is continuous and therefore the semantics of the while loop is well defined (which otherwise would not be immediate as the semantics of a while loop is defined as a least fixed point).
%
%
%
%
In the following section, we prove the soundness of the $\eetsymbol$ transformer with respect to an operational model.
